Adversarial Coordination on Social Networks

Decentralized coordination is one of the fundamental challenges for societies and organizations. While extensively explored from a variety of perspectives, one issue which has received limited attention is human coordination in the presence of adversarial agents. We study this problem by situating human subjects as nodes on a network, and endowing each with a role, either regular (with the goal of achieving consensus among all regular players), or adversarial (aiming to prevent consensus among regular players). We show that adversarial nodes are, indeed, quite successful in preventing consensus. However, we demonstrate that having the ability to communicate among network neighbors can considerably improve coordination success, as well as resilience to adversarial nodes. Our analysis of communication suggests that adversarial nodes attempt to exploit this capability for their ends, but do so in a somewhat limited way, perhaps to prevent regular nodes from recognizing their intent. In addition, we show that the presence of trusted nodes generally has limited value, but does help when many adversarial nodes are present and players can communicate. Finally, we use experimental data to develop a computational model of human behavior, and explore a number of additional parametric variations, such as features of network topologies, using the resulting data-driven agent-based model.

==> Simulations.tex <==
\section{Model}
We consider a social network between a group of players, in which some players are considered friends and can communicate.... . This social network is represented as graph  $ G = (V,E) $ with a vertex $ v \in V $ for each player and undirected edge $ e \in E $ from $ v_i $ to $ v_j $ for any two players $ (v_i,v_j) $ that have a way of communicating. 

\section{Baseline Strategies}
We begin our evaluation with a simulation of a fully-rational players' behavior in such networks, when aiming to reach a consensus. We do so by providing the players with two possible strategists, \emph{Majority} and \emph{Follow the leader}. In the \emph{Majority} strategy, a player choose her action (i.e., color) based on the majority of colors she observes by her neighbors.~\footnote{As a tie-break rule, players add their own current color and decide based on the updated majority.} The  \emph{Follow the leader} strategy is applicable in case one of the player's neighbors is a visible node. In this case, the player chooses the same color chosen by the visible node.
When testing the promise of visible nodes in this simulated framework, we were surprised  by the results reported in Table~\ref{tab:noInitial}. 
\begin{table}[hbt]
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline 
		v & 0 & 1 & 2 & 5 \\ 
		\hline 
		Ratio & 0.245  & 0.167 & 0.175 & 0.195 \\ 
		\hline 
	\end{tabular}  
	\caption{Visible nodes' effect on coordination} \label{tab:noInitial}
\end{table}
The maximal ratio of coordination is achieved without any visible node and there is a monotonic increase when the number of visible nodes increase from $ 1 $ to $ 5 $. Extensive analysis of the results lead to the insight that this results is due to the fact that the visible nodes did not have sufficient time to establish a stable ground of nodes that will broadcast the visible nodes' colors to the nodes that are not directly connected to them. Thus, we set a delay, denoted $ D $, that indicate the first time step in which nodes that are not connected to a visible node can take action. Any time step between $ 0 $ to $ D-1 $ is considered as a ``calibration'' step. Figure~\ref{fig:DelaySim} provides with the coordination ratio for graphs with $ 0 $, $ 1 $, $ 2 $ and $ 5 $ visible nodes for different values of $ D $. From $ D=12 $ and on, it is shown that visible nodes increase the ratio. Thus, we conclude that visible nodes can increase the ratio of successful coordination but only after initial time in which they calibrate their surroundings.
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{delay}
	\caption{REPLACE WITH A PYTHON FIGURE}
	\label{fig:DelaySim}
\end{figure}
